Integrated Approximate Dynamic Programming and Equivalent Consumption Minimization Strategy for Eco-Driving in a Connected and Automated Vehicle

This paper focuses on the velocity planning and energy management problems for Connected and Automated Vehicles (CAVs) with hybrid electric powertrains. The eco-driving problem is formulated in the spatial domain as a nonlinear dynamic optimization problem, in which information about the upcoming speed limits and road topography is assumed to be known a priori. To solve this problem, a novel Dynamic Programming (DP) based optimization method is proposed, in which a causal Equivalent Consumption Minimization Strategy (ECMS) is embedded. The underlying vehicle model to predict energy consumption over real-world routes is validated using experimental data. Further, a multi-layer hierarchical control architecture is proposed as a pathway to real-time implementation in a vehicle. The DP-ECMS algorithm is introduced for a long-horizon optimization problem, and then adapted for a receding horizon implementation using principles in Approximate Dynamic Programming (ADP). This computationally economical alternative to the traditional DP solution is then benchmarked and evaluated.

==> computation.tex <==
\section{Computational aspects of DP-ECMS}

Improving computation time of DP is relevant for frequent update of the velocity 
profile which is important if road and traffic conditions are changing. Especially if information is available through V2X or V2V communication \cite{grumert2017using}. Therefore, 
it is necessary to investigate different methods of reducing computation 
time of the DP-ECMS algorithm. 

\subsection{Parallelization of the DP algorithm}

The computations of the DP algorithm at each distance step can be 
parallelized since they are not depending on each other. If there are infinite 
resources for parallel computations, the lower bound of the total computational 
time is proportional to the time it takes to evaluate the system model times $T$.

Some experiments on parallelization of the DP algorithm has been conducted 
on a computer with 12 cpus where each cpu has two cores. Fig.~\ref{fig:cpu_time_par} 
shows the computation time as a function of the number of cores. 
When the computations are distributed on one core on each of the 12 cpus, the 
computation time is reduced by $50\%$ when doubling the number of cpus. When 
multiple cores are used on each cpu, the improvements are not as significant.

\begin{figure}
  \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {
      \resizebox{1\columnwidth}{!}{\includegraphics{Figures/cpu_time_par}}
    };
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
    \end{scope}
  \end{tikzpicture}
  \caption{Computational time of DP-ECMS as a function of number of cores on a computer with 12 cpu with 2 cores each. Computation time is cut by half each time the number of cpu doubles. When multiple cores are used on each cpu the computational time is reduced but not as fast.}
  \label{fig:cpu_time_par}
\end{figure}

%The computational time of DP is proportional to the number of evaluations 
%of the model, which is approximately $N_x N_u N_s$ where $N_x$ is the number of combinations 
%of the state variables, $N_u$ is the number of combinations of input 
%variables, and $N_s$ is the number of discretization steps of the route.
%Assuming that the number of state variables and input variables are fixed, 
%one of the first steps is to tune the level of discretization of the state and input 
%variables such that a satisfactory trade-off between computation time and 
%solution accuracy is achieved. A second case is considered here investigating 
%two approaches of reducing $N_s$ by using variable 
%discretization steps and reduced distance horizon. The third case does not reduce 
%the computational complexity but utilizes that parts of the computations can be 
%parallelized to reduce computational time.

% \subsection{Variable distance step discretization} 

% Discuss and analyze the effects of variable discretization of distance steps. 

\subsection{Look-ahead interval analysis}

Instead of computing DP of the whole route, a limited distance can be used, similar to MPC.

Discuss and analyze the effects of distance horizon in DP-ECMS.

==> problem.tex <==
\section{Optimization Problem Formulation}
\label{sec::problem}

The objective of the nonlinear dynamic optimization formulated is to minimize the fuel consumption of the vehicle over the entire driving mission. This problem is cast in the spatial domain to simplify the process of incorporating position-based route information.

The global optimization is now formulated over the full-route comprising of $N$ discrete grid points. Consider a discrete-time dynamic system in the form:
\begin{equation}
x_{k+1} = f_k(x_k,u_k) \quad k = 1, \ldots, N-1     
\end{equation}
where $k$ is the grid point along the route, and the dynamic states $x_k$ and control inputs $u_k$ are discrete variables. The state variables used in the model are the energy (or more precisely, the square of the vehicle velocity, $v_{veh,k}^2$) and the battery SoC ($\xi_k$). One of the key benefits of using the energy as the state instead of the velocity is that the simple Euler forward method can be used with adequate solution characteristics, as discussed in \cite{hellstrom2010design}. The engine brake torque ($T_{eng,k}$) and BSG torque ($T_{bsg,k}$) are chosen as the control variables. The optimization states and control actions are summarized as follows:
\begin{equation}
\begin{aligned}
x_k = \begin{bmatrix}
v_{k}^2 \\
\xi_k
\end{bmatrix} \in \mathcal{X}_k \subset \mathbb{R}^2,
\hspace{0.5cm}
u_k = \begin{bmatrix}
T_{eng,k} \\
T_{bsg,k}
\end{bmatrix} \in \mathcal{U}_k \subset \mathbb{R}^2
\label{eq::states_inputs_DP}
\end{aligned}
\end{equation}
The function that constrains the control and the state, $h_k: \mathcal{X}_k \times \mathcal{U}_k \to \mathbb{R}^r$ is expressed as $h_k(x_k,u_k) \leq 0, \forall k = 1, \dots, N-1$. Specifically, the constraints of the $N$-step optimization are:
\begin{equation}
\label{eq::prb_constr_opt}
\begin{aligned}
v_{k} &\in \left[v_{k}^{min}, v_{k}^{max} \right], \quad \forall k = 2, \dots, N \\
\xi_k &\in \left[\xi^{min}, \xi^{max} \right], \quad \forall k = 2, \dots, N \\
v_1 &= v_1^{min}, \quad \xi_1 \in \left[\xi^{min}, \xi^{max} \right] \\
a_k &\in \left[a^{min}, a^{max} \right], \quad \forall k = 2, \dots, N \\
T_{eng,k} &\in \left[T_{eng,k}^{min}\left(v_k \right), T_{eng,k}^{max}\left(v_k \right) \right], \forall k = 1, \dots, N-1 \\
T_{bsg,k} &\in \left[T_{bsg,k}^{min}\left(v_k \right), T_{bsg,k}^{max}\left(v_k \right) \right], \forall k = 1, \dots, N-1
\end{aligned}
\end{equation}
where, $v_{veh}^{min}$ and $v_{veh}^{max}$ are the minimum and maximum route speed limits respectively; $\xi^{min}$ and $\xi^{max}$ represent the static limits applied on battery SoC variation; $T_{eng}^{min}$ and $T_{eng}^{max}$ are the state-dependent minimum and maximum torque limits of the engine respectively, and $T_{bsg}^{min}$ and $T_{bsg}^{max}$ are the state-dependent minimum and maximum BSG torque limits respectively. To ensure SoC-neutrality over the global optimization, a terminal constraint is applied on the battery SoC: $\xi_1 = \xi_N$. Further, dynamical constraints are imposed by the vehicle model dynamics, described in Equations \ref{eq::engine_model_T_eng_fuel} - \ref{eq::longitudinal_dyn_model}.

%An admissible control map at grid point $k$ is a map $\mu_k : \mathcal{X} \to \mathcal{U}$ such that $h(x,\mu_k(x)) \leq 0, \forall x \in \mathcal{X}$. The collection of admissible control maps, $\mathcal{M} := \left(\mu_{1}, \dots, \mu_{N-1} \right)$ is referred to as the control policy. The controller aims at minimizing a cost, given by:
%\begin{equation}
%\label{eq::prb_cost_fn_gen}
%\begin{aligned}
%J(\mathcal{M}) = g_N(x_N) + \sum_{k = 1}^{N-1} g_k(x_k,u_k)
%\end{aligned}
%\end{equation}
%where, $c_k : \mathcal{X}_k \times \mathcal{U}_k \to \mathbb{R}$ is the arc (or stage) cost function, considered in this approach as a weighted average of the fuel consumption and travel time:
%\begin{equation}
%\label{eq::prb_cost_fn}
%\begin{aligned}
%g_k(x_k,u_k) = \left(\gamma \cdot \frac{\dot{m}_{f,k}(x_k,u_k)}{\dot{m}_f^{norm}} + (1-\gamma)\right) \cdot t_k \\
%\end{aligned}
%\end{equation}
%where, $\gamma$ is a tuning parameter that represents driver aggressiveness by penalizing the travel time, $\dot{m}_{f,k}$ is the fuel consumption rate, $\dot{m}_f^{norm}$ is a cost normalizing factor and $t_k$ is the per stage travel time.



